Evaluating Computational Language Models with Scaling Properties of Natural Language

In this article, we evaluate computational models of natural language with respect to the universal statistical behaviors of natural language. Statistical mechanical analyses have revealed that natural language text is characterized by scaling properties, which quantify the global structure in the vocabulary population and the long memory of a text. We study whether five scaling properties (given by Zipf's law, Heaps' law, Ebeling's method, Taylor's law, and long-range correlation analysis) can serve for evaluation of computational models. Specifically, we test $n$-gram language models, a probabilistic context-free grammar (PCFG), language models based on Simon/Pitman-Yor processes, neural language models, and generative adversarial networks (GANs) for text generation. Our analysis reveals that language models based on recurrent neural networks (RNNs) with a gating mechanism (i.e., long short-term memory, LSTM; a gated recurrent unit, GRU; and quasi-recurrent neural networks, QRNNs) are the only computational models that can reproduce the long memory behavior of natural language. Furthermore, through comparison with recently proposed model-based evaluation methods, we find that the exponent of Taylor's law is a good indicator of model quality.

==> later.tex <==
\section{Evaluation of Metrics}
\label{sec:evalmetrics}
Remind that we are interested in the two interdependent topics.
\begin{itemize}
	\item Whether the scaling properties and other evaluation metrics really evaluate the quality of text.
	\item Whether the language models reproduce the scaling properties of natural language that is present in dataset.
\end{itemize}
In this section, we focus on the first question and discuss the second question in the next section.
We regard the perplexity of language model as a measure of quality of text.
If the results of evaluation metrics have positive correlation with the perplexity of language model and is the best for the dataset, we consider the metrics can fairly evaluate the quality of text.

The first column of \tabref{tab:summary-WT2} and \tabref{tab:summary-PTB} lists the perplexity of the language models. 
The blank symbol ``-'' appears for the dataset, shuffled dataset, mathematical models and grammatical models because we cannot well-define perplexity for these models. 
Precisely, although it is possible to compute perplexity for these models, 
the values are not compatible because the PCFG generates text in tree-form and the mathematical models do not make prediction.

As it has been reported, the neural language models consistently outperform the $n$-gram models. 
Among $n$-gram models, Kneser-Ney smoothing consistently outperforms other smoothing techniques. 
3-gram models often has better perplexity over 5-gram models as the datasets in the experiment are not extremely large 
(roughly 1 million tokens).
The family of AWD-LSTM significantly improves their performance over the LSTM that is not regularized.
As it has been reported in various literature, regularization is crucial for the performance of language models.
The cache architecture and mixture of softmax also improve perplexity of the AWD-LSTM.

\subsection{The best scaling properties for evaluation}
The rest columns of \tabref{tab:summary-WT2} and \tabref{tab:summary-PTB} are the scaling properties, 
Zipf's law, Heaps' law, Ebeling's method, Taylor's law and long-range correlation.
Overall, the all scaling properties except for long-range correlation are robust to dataset.
When it appears in one dataset, then it also appears in the other dataset. 
Further, it is possible to compute the scaling properties regardless of the types of language models or models of natural language.
The Zipf's law is satisfied by all the language models and the models of natural language. 
We indicate the presence of Zipf's law by ``Yes'' due to the reason stated in \secref{sec:zipf}.
The all language models also satisfy Heap' law. Because Heaps' law is a derivative of Zipf's law, this result is clear.
Because these properties can be acquired even with uni-gram language model, it is not a challenge for the models to accomplish Zipf's law and secondary Heaps' law.
Despite its fame, Zipf's law and Heaps' law have no capacity in evaluating the quality of language model and models of natural language. 

On the contrary, the rest scaling properties of long-range dependence can evaluate the quality of text.
Three properties, Ebeling's fluctuation analysis, Taylor's law and the auto-correlation function have a reasonable correspondence. When the long-range dependence is detected from one method, the other methods also detect the long-range dependence.

Ebeling's fluctuation analysis quantifies the presence of long-range dependence in dataset and neural language models and its absence in the rest. 
The exponent of the datasets is 1.32 in WT2 and 1.23 in PTB whereas that of the shuffled datasets is 1.0.
The results indicate the presence of long-range dependence in the dataset and absence in the shuffled datasets.
The exponent of the language models ranges between 1.0 and the values of the datasets.
The neural language models records between 1.10 and 1.30 for WT2, whereas between 1.04 and 1.13 for PTB.  
I contrast, the other language models were the same as i.i.d.  
Ebeling's method does have a certain level of capability to evaluate models.
It quantifies the qualitative difference the neural language models and the other models.
However, the correlation with the perplexity is not adequate. 
Plus, the Ebeling's method can be applied for sequence of character and not for that of word.
It limits the application of this method to evaluate the mathematical models such as Simon and Pitman-Yor process as they do not have a concept that connects to character.
Further, because the majority of language modeling use word-level modeling, the use of this character-based analysis is not straightforward.

The last column shows the results of the long range correlation.
If the text is not long-range correlated, this is mentioned by ``No'' or ``Weak'': ``No'' if more than one value was negative for $s\leq10$, or ``Weak'' for one negative value for $s\leq100$.
It also has a good correspondence with Ebeling's method  and Taylor's law.
One significant difference of this method is the detection of long memory in Simon model.
Simon model is a simple mathematical model and is unlikely to well resemble the human's linguistic activities.  
For the Simon model, the Taylor exponent was 0.5, indicating the absence of the clustering behavior.
Another problem lies in the values of exponent that seems be less correlating with Perplexity.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.8\textwidth]{figs/bars}
  \caption{Negative log-likelihood of PCFG (top), Perplexity computed with AWD-LSTM (2nd top), Taylor's  exponent(3rd top) and Perplexity(bottom) of WT2, its shuffled text and the models. Unmeasurable values are present as blank.}
  \label{fig:bars}
\end{figure}

The remaining Taylor's law seems the most reliable among the three scaling properties
The strength of Taylor's law is two fold: the Taylor's exponents have
positive correlation with perplexity and the exponent is
interpretable. \figref{fig:bars} shows the values of the Taylor's
exponent and perplexity for every language model.  
\figref{fig:bars} indicates that they are correlated well with differences for the most advanced neural language models.
It highlights some aspects of the model characteristics.

Overall, the scaling properties of long-range dependence can serve for evaluating the quality of text, and the models.
The famous Zipf's law and Heaps' law are not effective as they could be readily reproduced by the all models.
Among the scaling properties, Taylor's law and Taylor exponent are the most robust and have a good correlation with perplexity.

\subsection{Comparison with the PCFG and the language model based evaluation}
Among the scaling properties, the Taylor's law is the most robust and Taylor exponent have a reasonable positive correlation with perplexity of language models. 
We compare the Taylor's law with the negative log-likelihood of PCFG \cite{Subramanian_2017} and perplexity computed from neural language model \cite{Fedus_2018}, the two probable evaluation metrics that only require generated text.

The use of the PCFG is intuitively a straightforward and promising method for evaluating the grammaticality of text.
The PCFG should be ideally capable of distinguishing the syntactically correct and wrong sentences.
However, the PCFG in fact have poor evaluation performance. 
The values in the third column of \tabref{table:eval_WT2} and \tabref{table:eval_PTB} fluctuate around 35 for any dataset, 
shuffled dataset and the texts generated from a wide range of language models. 
Appendix 2 presents further details to clarify the inability of the PCFG.
We cannot use the PCFG for fair evaluation of generated text.

\citet{Fedus_2018} proposed to evaluate the quality of generated text with the perplexity computed from neural language model.
This approach is a straight application of language model and is working as expected to a certain level.
The rightest column of \tabref{table:eval_WT2} and \tabref{table:eval_PTB} is the perplexity of text computed by AWD-LSTM.
The neural language model can distinguish the difference among the $n$-gram language models, neural language models and dataset.
We should however note that the interpretability of the result is limited in two points.
First, in the $n$-gram language models, Katz backoff models perform the best in the computed perplexity while Kneser-Ney is the best model.

\figref{fig:bars} presents the three evaluation metrics, Taylor exponent, the negative log likelihood of PCFG and perplexity of AWD-LSTM, a neural language model with respect to the perplexity of the language models.
We find that the PCFG is useless for evaluating text and Taylor exponent and neural language model can be fair evaluation metrics.
We should note that the use of neural language model limits interpretability of the result and the relatively high evaluation to the shuffled datasets rises question to the validity.
Taylor exponent has a strong positive correlation with perplexity. 
The method does detect the long-range dependence in the dataset and the best performing neural language models and never detect it in the shuffled datasets and $n$-gram models.

\begin{figure*}[t]
  \twofig{AWD_LSTM_Cache_WT2_word_line}
%\vspace*{-0.5cm}
\caption{Scaling properties of AWD-LSTM-Cache model trained with WT2. 
\label{fig:awdcache}}
\end{figure*}


\section{Evaluation of the models}
\label{sec:evalmodels}

Finally, we discuss the quality of the models with scaling properties.
We are interested in the scaling properties of the language models and models of natural language 
because they are universal to natural language and language-related data. 
All language models in the experiment satisfy the scaling properties of vocabulary population, Zipf's law and Heaps' law.
They are easy for the models to reproduce because they are about the static probability distribution. 

On the contrary, the all language models except neural language models fail to reproduce the long-range dependence.
The other $n$-gram models and the PCFG show same behavior from this perspective.
They totally fail to reproduce the long range dependence of natural language. 
The lack of long memory in $n$-gram language model can be supported by theoretical analysis on Markov model.
From various approaches, it has been proved that a Markov model has a short memory and does not have a long memory.
The failure of PCFG can be explained with the lack of inter-sentence structure in the model.
Taylor's law quantifies the universal structure other than syntax and is about the long-ranged, beyond sentence structure.
The sole exception was the mathematical model, Simon model which presented strong long-range correlation, even stronger than that of the original WT2.  
However, its Taylor exponent is 0.5 that implies the absence of long-range dependence.
This analysis reveals that the Simon model is not sufficient for describing the fundamental statistical properties of natural language.

In contrast, for the neural language models were able to reproduce all of the scaling properties at different degrees.
\figref{fig:awdcache} shows a set of graphs for the AWD-LSTM-Cache model for WT2.
The figure shows how well the model captures the nature of the original text.
The size of the point cloud increases quantifying the presence of burstiness in the text and the language models.
The Taylor exponent for {\it Wikipedia} is 0.62, which indicates that the text has a temporal structure. 
For the $5$-gram language model, however, the exponent is 0.5, which corresponds to the i.i.d.
case, as mentioned before. This result suggests one critical limitation of $n$-gram 
models: they cannot maintain the presence of co-occurrence and burstiness in text, 
which are universally observed in human linguistic behaviors. In fact, all language 
models developed before deep learning have a Taylor exponent of 0.5.

Our analysis with Taylor's exponent further clearly quantify the possibility to improve the neural language models further.
The best performing AWD-LSTM-Cache model has Taylor exponent $\zeta$ of 0.59 which is smaller than the original text 0.62.
The cloud in Taylor's law of AWD-LSTM-Cache is noticeably smaller than that of the original dataset.
The neural language model can be improved through enhancing long range dependence.
This could be done through further memory augmentation structure of neural networks.

\begin{figure}[h]
	\twofig{image_coco_shuffle_word_line}
	\vspace*{-0.5cm}
 \caption{Scaling properties of captions in image coco dataset. \label{fig:coco}}
 	\twofig{seq_word_line}
 \caption{Scaling properties in captions generated by Seq-GAN}
 \end{figure}

\section{Discussion: on the evaluation of GAN models}
We have introduced three metrics to evaluate quality of text without reference and without access to probability distribution.
The perplexity computed from the PCFG is perfectly useless. The evaluation with neural language model is fair, 
but remains difficult to interpret the significance of the result.
The rest, metrics that derive from scaling properties and the are generally able to evaluate the quality of the language models without reference.
It motivates us to evaluate the GAN generated text with the scaling properties.

\figref{fig:coco} shows the two representative scaling properties of the ImageCoco dataset \cite{Lin_2014} and the generated captions from Seq-gan \cite{Yu_2017}. 
Zipf's law is present in the dataset.
Unlike the models of natural language presented so far, the GAN models have problems in reproducing Zipf's law.
The decay in the generated text is significantly faster than the decay in the dataset.
It indicates that the GAN model is not capable of generating a wide range of vocabulary or is model-collapsed.
In the works such as \cite{Yu_2017,Guo_2017,Fedus_2018}, the model-collapse is investigated through the use of BLEU explained in Section 2.
Zipf's law is another method to inspect the model-collapse.	

The long-range dependence is absent as the caption dataset is a collection that has no dependence between entries.
Taylor exponent is 0.5 for the image captions that are shuffled by caption and is how the captions are generated from the model 
as the captions are essentially independent each other.
The application of the long-range dependence based analysis is not well suited for the current GAN research. 
The long-range dependence analysis literally requires the models to generate sufficiently long text.
Instead, the perplexity of text computed from neural language model may provide a reasonable assessment on the quality of text.
However, because the fundamental motivation towards the GAN and other generative models is the replication of complex phenomena in the world, 
the studies aim and accomplish to model the scaling properties of natural language as they are universal and complex structure.

\section{Conclusion}
In this paper, we explored the evaluation of machine generated text with the scaling properties of natural language.
The scaling properties such as Taylor's law and long-range correlation are universal to the genre and language of text 
and they can quantify the long-range dependence in text.
We demonstrated that such scaling properties can be feasible and actually desirable evaluation metrics of natural language.
They have a reasonable positive correlation with perplexity, the primary metrics of language model. 
Among the scaling properties, the Taylor's law performs the most robust. 
Taylor's exponents can quantify the degree to which the models reproduce the long-range dependence in text and show a reasonable correlation with perplexity of the language models. 
Through the analysis, we quantified that the state of the art neural language models and the other $n$-gram models and the PCFG are qualitatively different. 
The neural language models capture the long-range dependence of text that $n$-gram language models and the PCFG never reproduce.

In addition to the scaling properties, we demonstrated that the evaluation of quality of text remains meaningless or at least  questionable.
We specifically show that the PCFG does not correlate with the quality of text at all. 
Even the negative log-likelihood of shuffled datasets is equivalent to the original dataset.
The perplexity computed from a neural language model provide a rough judge to the quality of text. However the fluctuation of the value is relatively large and is less reliable to the scaling properties. 


==> table.tex <==
%
%\begin{table}[h]
%  \caption{The statistics of dataset used in this article: \textcolor{red}{WOULD YOU PLEASE MAKE THIS TO INCLUDE
%      EXPONENTS JUST LIKE THE TWO TABLES 2,3}}
%\label{tab:nldata}
%  \begin{tabular}{lllll}
%\hline
%  text & language & vocabulary & length & note \\
%\hline
%Shakespeare&English&&&collection\\
%HongLouMeng&Chinese&&&\\
%Wikitext2 & English & & & \\
%PennTree Bank & English & & &  \\
%ImageCoco & English & & & Standard dataset for GAN\\
%\hline
%\end{tabular}
%\end{table}


  \begin{tabular}{|l||c|c|c|c|c|c|c|}
    \hline
    &  Tokens & Vocab & \multicolumn{2}{|c|}{Vocabulary Population} & \multicolumn{3}{|c|}{Long Memory} \\ \cline{4-8}
   &  & -ulary& Zipf's & Heaps'  & Ebeling's & Taylor's & Long Range\\
   &&&Law&Law&Method&Law&Correlation\\
   &&&$f(r)\propto r^{-\alpha}$&$v(n)\propto n^\beta$  
   & $m(l) \propto l^{\eta}$&$\sigma \propto \mu^{\zeta}$ & $c(s) \propto s^{-\xi}$\\
    \hline
\multicolumn{8}{|c|}{Wikitext-2 (English, Wikipedia article)}\\\hline
  preprocessed dataset & 2,088,628   & 33,278 & Yes & 0.75 (0.13)& 1.33 (0.10)& 0.62 (0.15) & 0.33 (0.04) \\ \hline
original dataset & 2,088,628 & 76,617  & Yes& 0.78 (0.09)& 1.33 (0.10) & 0.65 (0.11) & 0.32 (0.03) \\
    \hline
    \multicolumn{8}{|c|}{Penn Treebank (English, The Wall Street Journal news article)} \\
    \hline
 preprocessed dataset & 887,521 & 10,000 & Yes & 0.70 (0.16) & 1.23 (0.06) & 0.56 (0.14) & 0.81 (0.24)   \\ \hline
 original dataset & 892,008   & 89,317  & Yes & 0.83 (0.07)& 1.20 (0.05)  & 0.57 (0.06) & 0.60 (0.16) \\   
    \hline
    \multicolumn{8}{|c|}{Shakespeare (old English collection of literature works)} \\
     \hline
   original text  & 740,706 &  83,105 &  Yes &  0.79 (0.07) &  1.24 (0.09) & 0.59 (0.05) & 0.13 (0.02) \\
   \hline
 \multicolumn{8}{|c|}{Hong Lou Meng (Chinese, literature work)} \\
      \hline
original text & 703,034 & 18,312 & Yes  & 0.74 (0.14)   & 1.31 (0.07) & 0.58 (0.07)  & 0.39 (0.04) \\
\hline
%%     \multicolumn{8}{|c|}{Image COCO (English, collection of image caption)} \\
%%  \hline
%% \begin{tabular}[l]{@{}l@{}}original dataset\\ (sorted by category)\end{tabular} & 105,933   & 6,095 &Yes & 0.76 (0.08) &   1.08 (0.05)  & 0.55 (0.06)                                                & 0.35 (0.34) \\ \hline
%% \begin{tabular}[l]{@{}l@{}}original dataset\\ (shuffled by caption)\end{tabular} & 105,933   & 6,095  & Yes & 0.76 (0.09) &  0.99 (0.03)  & 0.50 (0.04)                                                & No \\
%\hline
   \end{tabular}


